Phase space density limitation in laser cooling without spontaneous emission

We study the possibility to enhance the phase space density of non-interacting particles submitted to a classical laser field without spontaneous emission. We clearly state that, when no spontaneous emission is present, a quantum description of the atomic motion is more reliable than semi-classical description which can lead to large errors especially if no care is taken to smooth structures smaller than the Heisenberg uncertainty principle. Whatever the definition of position - momentum phase space density, its gain is severely bounded especially when started from a thermal sample. More precisely, the maximum phase space density, can only be improved by a factor M for M-level atoms. This bound comes from a transfer between the external and internal degrees of freedom. To circumvent this limit, one can use non-coherent light fields, informational feedback cooling schemes, involve collectives states between fields and atoms, or allow a single spontaneous emission even

==> SM.tex <==



\title{Supplemental Material for \\ Phase space density limitation in laser cooling without spontaneous emission}
\author{Thierry Chaneli\`{e}re, Daniel Comparat and Hans Lignier}
\affiliation{Laboratoire Aim\'{e} Cotton, CNRS, Univ. Paris-Sud, ENS Paris Saclay, Universit\'e Paris-Saclay, B\^{a}t. 505, 91405 Orsay, France}

\date{\today}
\maketitle

\onecolumngrid



\section{Non-relativistic Hamiltonian of non-interacting particles}

We here recall the equations of motion for laser cooling of atoms. The reader can refer to textbooks such as 
\cite{CDG2}.


\subsection{Quantized or (semi-)classical hamiltonian}

We  here study the quantum Hamiltonian $\hat H$ of a two generic levels $|1\rangle$ and $|2\rangle$ (representing the ground $|g\rangle$ and the excited $|e\rangle$  states in \cite{main_art}) of a particle (mass $m$) under the effect of electromagnetic fields. The generalisation to $M$ level system is straightforward but will not be detailed for the sake of simplicity. We separate the "motional" (or trapping) fields that do not couple $|1\rangle$ and $|2\rangle$, such as trapping potential $V_1,V_2$  produced for example by magnetic coils, magnets or electrodes through Zeeman  ($-\hat{\bm \mu} . \bm B$) or   Stark effect ($-\hat{\bm d}.\bm E$), and the laser fields $\hat{\bm E}$  that do couple $|1\rangle$ and $|2\rangle$. 

For $N$  non-interacting particles the full hamiltonian can be written as
$\hat H=  \sum_{i=1}^N \hat H^{(i)} + \hat H_{\rm field} + \sum_{i=1}^N \hat H_{\rm int, field}^{(i)} $, where $\hat H^{(i)}$ is the hamiltonian $\displaystyle \frac{\bm \hat p_i^2}{2 m} + 
V_1(\hat{\bm r}_i,t) |1\rangle\langle 1| + V_2(\hat{\bm r}_i,t) |2\rangle \langle 2|$ for the position and momentum $\bm p_i,\bm r_i$ of the $i^\mathrm{th}$ particle. The trapping field is arbitrary but the simplest case corresponds to harmonic traps: $V_i = E_i +\frac{1}{2} m \omega_i \bm r^2$. A base of the Hilbert space will be an ensemble of states $\displaystyle \bigotimes_{i=1}^{N} |\bm p_i,1\ {\rm or} \ 2\rangle_i \otimes | \Uppi_{\bm{k} \sigma}  n_{\bm{k} \sigma} \rangle$ when using the Fock notation for the field.
We treat the $N$ particles as totally independent  and use the 
density matrix formalism (written as $\hat \rho$) to describe the system of $N$ identical particles as a statistical ensemble. The external field is common to the $N$ atoms and this can automatically generate entanglement between the atoms or collective behaviour  that can indeed lead to cooling \cite{beige2005cooling,vacanti2009cooling}. 
As explained in the article, this is not our interest here and we shall study only the single particle case.
In the dipolar approximation and neglecting the 
Roentgen term, despites the fact  that it can create surprising radiation forces  on the atoms \cite{barnett2017vacuum,2017arXiv170401835S},
the Hamiltonian for a single particle reads as:
\begin{equation}
\hat H =  \frac{\hat{\bm p}^2}{2 m} + 
V_1(\hat{\bm r},t) |1\rangle\langle 1| + V_2(\hat{\bm r},t) |2\rangle \langle 2| \label{eq_base_at}
 -  \bm d. \hat{\bm E} (\hat{\bm r} ,t) (   |2\rangle \langle 1| + |1\rangle \langle 2| ) +
\sum_{\bm{k} \sigma} \hbar \omega_k \left( \hat a^\dag_{\bm{k} \sigma} \hat a_{\bm{k} \sigma} + 1/2 \right) 
\end{equation}
where $\bm d$ is the transition dipole element  (assumed to be real $\bm d = \langle 2 | q \hat {\bm r}| 1 \rangle $) and
 $\hat{\bm E} (\bm r ,t)$ is a quantized real field. For instance for a single plane wave field (in a volume $L^3$)
$\displaystyle	\hat{\bm{E}} (\bm{r},t)  = \sum_{\bm{k},\sigma} i \sqrt{\frac{ \hbar  \omega_k}{2  \epsilon_0 L^3} } \left(  \hat a_{\bm{k} \sigma} e^{- i \omega_k t}  \bm{\epsilon}_{\bm{k}\sigma} {\rm e}^{i \bm{k}.\bm{r} }  - \hat a_{\bm{k} \sigma}^\dag  e^{ i \omega_k t}  \bm{\epsilon}_{\bm{k}\sigma}^\ast {\rm e}^{-i \bm{k}.\bm{r} } \right)$. %The trapping field are arbitrary but the simplest case corresponds to harmonic traps: $V_i = E_i +\frac{1}{2} m \omega_i \bm r^2$.

%A base of the Hilbert space, for a given atom, is 	an ensemble of states $ |\bm p\rangle \otimes |1\ {\rm or} \ 2\rangle \otimes | \Uppi_{\bm{k} \sigma}  n_{\bm{k} \sigma} \rangle$ when using the Fock notation for the field.

The initial state is uncorrelated and  density operator can be written as an atomic (external and internal degrees of freedom) and a field part as
$\displaystyle \hat \rho = \hat{\rho}_{\rm at} \otimes \hat{\rho}_{\rm field} =  \hat{\rho}_{\rm ext} \otimes  \hat{\rho}_{\rm int} \otimes  \hat{\rho}_{\rm field}  $.


In the semi-classical approximation, we would like to replace the field operators (denoted with the hat $ \hat{}  $ ) by their classical expectation values, namely
$\hat a_{\bm{k} \sigma}$ and $\hat a_{\bm{k} \sigma}^\dagger$ by c-numbers
$ a_{\bm{k} \sigma}$ and $ a_{\bm{k} \sigma}^*$, such as 
	$ \hat{\bm E} (\hat{\bm r} ,t)$ by $   \bm E (\hat{\bm r} ,t)$
  becomes in the Hamiltonian
\begin{equation}
\hat H =  \frac{\hat{\bm p}^2}{2 m} + 
E_1(\hat{\bm r},t) |1\rangle\langle 1| + E_2(\hat{\bm r},t) |2\rangle \langle 2|
 - \bm d. \bm E (\hat{\bm r} ,t) (   |2\rangle \langle 1| + |1\rangle \langle 2| ) \nonumber \label{Hamil}
\end{equation}

\subsection{Classical fields}

This can be done, 
by using coherent states $|\alpha \rangle$,
that are eigenstates of the annihilation operator $\hat a$: $\hat{a}|\alpha\rangle=\alpha|\alpha\rangle$, by using the unitary transformation under the operator $\hat U =  \hat {\cal D}(\alpha_\lambda e^{-i\omega_\lambda } )^\dag $ and neglecting the quantum field that now describes  spontaneous emission only \cite{mollow1975pure,Cohen-Tannoudji1997,dalibardcoolegeFrance2015}.

%Because we neglect the spontaneous emission, we can use the Mollow prescription \cite{mollow1975pure}.
%that
%recovers, for coherent states, a pure classical field evolution.

Therefore, in the following
we assume  to have classical laser fields with different frequencies $\omega_{\rm L}$, wave-vectors ${\bm k}_{\rm L}$ or temporal phase $\Phi_{\rm L}(t)$:
${\bm E}(\hat{\bm r},t) = 
{\bm E'}(\hat{\bm r},t)+ {\bm E'}^\dag(\hat{\bm r},t) =
\frac{1}{2}\sum_{\rm L}    \left[ {\bm E}_{\rm L}(t) e^{i(  {\bm k}_{\rm L}. {\hat{\bm r}} - \omega_{\rm L} t   - \Phi_{\rm L}(t)
	)} +  {\bm E}_{\rm L}^\ast(t) e^{-i(  {\bm k}_{\rm L}. {\hat{\bm r}}  - \omega_{\rm L} t   - \Phi_{\rm L}(t)
	)}  \right] $.
The rotating wave approximation leads to

\begin{equation}
\hat H =  \frac{\bm \hat {\bm p}^2}{2 m} + 
V_1(\hat {\bm r},t) |1\rangle\langle 1| + V_2(\hat {\bm r},t) |2\rangle \langle 2| 
 -  \bm d .\bm E' (\hat {\bm r} ,t)  |2\rangle \langle 1| - \bm d .  \bm E'^\dag (\hat {\bm r} ,t)  |1\rangle \langle 2|) \label{hamiltonianRWA}
\end{equation}

We will now use this Hamiltonian to describe the evolution.
In matrix notation with the  $|1,2\rangle$ basis,  the Hamiltonian (\ref{hamiltonianRWA}) becomes
$\hat H = \begin{pmatrix}
\hat H_1 & \hat V^\dag \\ 
\hat V & 	\hat H_2
\end{pmatrix} $
where the coupling term is  $\displaystyle \hat V = -  \bm d .\bm E' (\hat r ,t) =
- \frac{\bm d}{2}\sum_{\rm L}    {\bm E}_{\rm L}(t) e^{i(  {\bm k}_{\rm L}. {\hat{\bm r}} - \omega_{\rm L} t  - \Phi_{\rm L}(t) )}		= \sum_{\rm L}	\hat V_{\rm L}	$.	




\subsubsection{Density matrix}


The time evolution 
$\displaystyle i \hbar \frac{\partial \hat \rho}{\partial t} = \hat H \hat \rho - \hat \rho \hat H$ leads to:
\begin{widetext}
	$ \begin{pmatrix}
	\frac{\partial \hat \rho_{11} }{\partial t}	 & 	\frac{\partial \hat \rho_{12} }{\partial t} \\ 
	\frac{\partial \hat \rho_{21} }{\partial t} & 	\frac{\partial \hat \rho_{22} }{\partial t}
	\end{pmatrix} = \frac{1}{i\hbar}
	\begin{pmatrix}
	[\hat H_1,\hat \rho_{11}]+ \hat V^\dag \hat \rho_{21} - \hat \rho_{12 } \hat V   & [\hat p^2/2m,\hat \rho_{12}] + \hat V_1 \hat \rho_{12} - \hat \rho_{12} \hat V_2 + \hat V^\dag \hat \rho_{22} - \hat \rho_{11} \hat V^\dag\\ 
	[\hat p^2/2m,\hat \rho_{21}] + \hat V_2 \hat \rho_{21} - \hat \rho_{21} \hat V_1 + \hat V \hat \rho_{11} - \hat \rho_{22} \hat V & 	[\hat H_2,\hat \rho_{22}]
	+ \hat V\hat \rho_{12} - \hat \rho_{21 } \hat V^\dag
	\end{pmatrix}
	$
\end{widetext}




\subsubsection{Wigner functions}

\onecolumngrid

The Wigner-Weyl transform of this equation gives the time evolution of the Wigner function defined as	
 

	\begin{equation}
	W(\bm r,\bm  p,t) = \frac{1}{h^3}
	\int \langle  \bm  p - \bm  p'/2 | \hat \rho (\hat{\bm  r},\hat{ \bm p}, t) | \bm  p + \bm p'/2 \rangle e^{-i \bm r.\bm  p'/\hbar} d\bm  p'  
	\end{equation}

through the so-called Moyal bracket, governed by

\begin{equation}	\frac{\partial W}{\partial t} =  \frac{1}{i \hbar} \left(H \star W - W \star H \right) \end{equation}

The  $\star$-product
can
be evaluated using the convenient formula
\cite{curtright2014concise} for any generic function $\rho_{1,2}(r,p)$
\begin{eqnarray*}
	(\rho_1 \star 	\rho_2) (r,p) &= & 	\rho_1(r+i\frac{\hbar}{2} \frac{\partial}{\partial p},p-i\frac{\hbar}{2} \frac{\partial}{\partial r}) 	\rho_2(r,p) \\
	(\rho_2 \star 	\rho_1) (r,p) &= & 	\rho_2(r-i\frac{\hbar}{2} \frac{\partial}{\partial p},p+i\frac{\hbar}{2} \frac{\partial}{\partial r}) 	\rho_1(r,p) 
\end{eqnarray*}
that we have restricted to a one dimensional motion for simplicity.

Therefore,
when no  $\hat r$, $\hat p$ product are present in $\hat \rho = \rho(\hat r, \hat p)$,
the  Wigner(-Weyl) transform $W_{\hat \rho}(r,p;t)$  is  the unmodified classical observable expression $\rho(r,p)$. An important example is a conventional Hamiltonian, $\displaystyle \hat H = \hat p^2/2m +V(\hat r,t)$, for which the transition from classical
mechanics  is the straightforward quantization: $\displaystyle W_{\hat H}(r,p;t) = H(r,p;t) = p^2/2m +V(r,t)$.

The expressions containing  $ e^{i  {\bm k}_{\rm L}. {\hat{\bm r}} }$
can be expanded by
using exponential (Taylor) series  that indicates	
$e^{i  { k}_{\rm L} \left(
	r \pm \frac{i  \hbar}{2}   \frac{\partial }{\partial  p}
	\right) } f(r,p,t) = 
e^{i   k_{\rm L} r} f(r,p  \mp   \hbar   k_{\rm L} /2   ,t)
$.
% which is nothing else that the well known translation operator $   e^{-i a \hat p/\hbar  } | r \rangle = | r + a \rangle $
and finaly using $\displaystyle \hbar \Upomega_{\rm L}(r,t) = 
\bm d. {\bm E}_{\rm L} e^{ i ( {\bm k}_{\rm L}. {\bm r}  - \omega_{\rm L} t  - \Phi_{\rm L}(t) )} $,
 we obtain:
	{\footnotesize
	\begin{eqnarray}
	\left[ \frac{\partial   }{\partial t}	 
	+\frac{ p}{m} \frac{\partial }{\partial  r}   
	- 
	\frac{1}{i\hbar}	[V_1(r+i\frac{\hbar}{2} \partial_p) - V_1(r-i\frac{\hbar}{2} \partial_p) ] \right]W_{11}(r,p,t) &= &  
	-
	\frac{1}{2 i} \sum_{\rm L} ( \Upomega_L^* (r,t)
	W_{21} (r,p+\frac{\hbar k_{\rm L}}{2},t) - \Upomega_L (r,t) W_{12} (r,p+\frac{\hbar k_{\rm L}}{2},t)
	) \label{Wigner_eq_brute_1}
 	\\
	\left[	\frac{\partial   }{\partial t}+\frac{ p}{m}  \frac{\partial }{\partial  r} 
	-
	\frac{1}{i\hbar}	[V_1(r+i\frac{\hbar}{2} \partial_p) - V_2(r-i\frac{\hbar}{2} \partial_p) ] \right] W_{12}(r,p,t) & = &
	-
	\frac{1}{2 i} \sum_{\rm L} \Upomega_L^* (r,t) (
	W_{2 2} (r,p+\frac{\hbar k_{\rm L}}{2},t) - W_{11} (r,p-\frac{\hbar k_{\rm L}}{2},t)
	)
	\label{Wigner_eq_brute_2}
	\\
	\left[	\frac{\partial   }{\partial t}  +\frac{ p}{m}  \frac{\partial }{\partial  r} 
	- 
	\frac{1}{i\hbar}	[V_2(r+i\frac{\hbar}{2} \partial_p) - V_1(r-i\frac{\hbar}{2} \partial_p) ] \right] W_{21}(r,p,t) & = &
	-
	\frac{1}{2 i} \sum_{\rm L} \Upomega_L (r,t) (
	W_{11} (r,p-\frac{\hbar k_{\rm L}}{2},t) - W_{22} (r,p+\frac{\hbar k_{\rm L}}{2},t)
	)
	\label{Wigner_eq_brute_3}
	\\	
	\left[	\frac{\partial  }{\partial t}
	+\frac{ p}{m}  \frac{\partial }{\partial  r}   
	-	\frac{1}{i\hbar}	[V_2(r+i\frac{\hbar}{2} \partial_p) - V_2(r-i\frac{\hbar}{2} \partial_p) ] \right]   W_{22} (r,p,t)   &=  &
	- \frac{1}{2 i} \sum_{\rm L} ( \Upomega_L (r,t)
	W_{12} (r,p-\frac{\hbar k_{\rm L}}{2},t) - \Upomega_L^* (r,t) W_{21} (r,p-\frac{\hbar k_{\rm L}}{2},t)
	) 
	\label{Wigner_eq_brute_4}
	\end{eqnarray}
	}
For completeness, we mention that a (1D) spontaneous emission rate $\Gamma$ can be added if needed, by including the terms \cite{dalibard1985atomic,1991JOSAB...8.1341Y}.

\begin{eqnarray*}
	\left.	\frac{\partial W_{11}}{ \partial t}	\right|_{\rm spon}  & =& \Gamma \int_{-p_r}^{p_r} \Theta(p') W_{22}(r,p+p') d p' \\
	\left.	\frac{\partial W_{11}}{ \partial t} 	\right|_{\rm spon}  & = &  - \frac{\Gamma}{2}  W_{12}(r,p)\\
	\left.	\frac{\partial W_{21}}{ \partial t} 	\right|_{\rm spon}  & = &  - \frac{\Gamma}{2}  W_{21}(r,p) \\	
	\left.		\frac{\partial W_{22}}{ \partial t} 	\right|_{\rm spon}  & = &  - \Gamma  W_{22}(r,p)
\end{eqnarray*}
where $\Theta(p')$ is the probability density distribution 
for 
the projection of spontaneous emission $\displaystyle \Theta(p')=  \frac{3}{8 p_r}\left(1 +\frac{p'^2}{p_r^2} \right)$ for a dipolar radiation pattern) on the atomic recoil momentum  for $ p_r = \hbar k$.


Equation of motion of the Husimi distribution can be derived \cite{lee1995theory,takahashi1989distribution,martens2011quantum,wyatt2006quantum,chattaraj2016quantum}
         and  present non-zero second term of the Liouville equation (similar to Eqs.(\ref{Wigner_eq_brute_1})-(\ref{Wigner_eq_brute_4}))


	
	
	
	\subsection{Connection with Liouville equation}
	
In the absence of light fields, Taylor series expansion indicates that the evolution of the diagonal terms $W_{ii}$ is  given by:
	\begin{equation*}
\frac{D W_{ii}}{D t} = 	\frac{\partial W_{ii}}{\partial t} + \frac{ p}{m} \cdot \frac{\partial W_{ii}}{\partial  r} - \frac{\partial V_i}{\partial  r}\cdot   \frac{\partial W_{ii}}{\partial  p}  = 
	 \sum_{s\geq 1} \hbar^{2s} \frac{2^{-2s}}{(2s+1)!} \frac{\partial^{2s+1} V_i}{\partial r^{2s+1} }
	\frac{\partial^{2s+1} W_{ii}}{\partial p^{2s+1} }
	\label{Wigner_evolution}
	\end{equation*}
	We recover the 
Liouville's equation, $\displaystyle \frac{D W_{ii}}{D t} = 0$, under the influence of the
	potential $V$, but only 
	for a quadratic potential $V_i(r,t) = a(t) + b(t) r +c(t) r^2$.
	However, when higher derivatives of $V_i(r)$ are present, additional terms will give rise to diffusion and the quantum Wigner function
	gradually deviates from the corresponding classical phase space probability density. So a non-harmonic potential is a clear way to modify the Wigner phase space density. This argument also applies to the Husimi function.




\subsection{Interaction picture: free evolution}	



The evolution  of $H_1(t)$ is given by the unitary time evolution operator 	$\hat U_1 (t) = e^{-i \int \hat H_1(t)/\hbar }$. 
In matrix notation, the		evolution operator is
$\hat U_0 = \begin{pmatrix}
\hat U_1 & 0 \\ 
0 & 	\hat U_2
\end{pmatrix} $.
The interaction picture consists in defining 
a new density matrix
$\displaystyle \hat \rho^I (t) = {\hat U_0}^\dag (t) \hat \rho (t) {\hat U_0} (t)$, which 
evolves under the
modified Hamiltonian 
$\displaystyle \hat H^I  = {\hat U_0}^\dag  \hat H {\hat U_0}  + i  \hbar \frac{d {\hat U_0}^\dag}{d t}   {\hat U_0}  =
\begin{pmatrix}
0 &{{\hat V}^I} {}^{\dag} \\ 
{{\hat V} {}^I} & 0
\end{pmatrix}$ where $\hat V^I = {{\hat U}_2}^\dag \hat V \hat U_1$.

Because several laser frequencies are possibly present, the interaction picture is more appropriate than the Bloch rotating frame. The latter would imply to choose one laser frequency as a reference. The interaction picture removes this arbitrariness.
%Bloch one because many lasers are presents. Indeed
% the rotating frame Bloch notation, which 
%multiplies coherences by terms $e^{\pm i \omega_L t}$, is simple only when a single laser frequency $\omega_L$ is present; wheras the interaction picture, that multiplies coherences by terms $e^{\pm i \omega_{ij} t}$, does not depends on the lasers and is efficient even when many laser are presents.

\subsubsection{Density matrix}
Using the momentum representation, where $\hat r$ acts as $i \hbar \partial_p$  on $ \psi(p) = \langle p | \psi\rangle$, we have 
$\displaystyle   e^{i k \hat r  } | p \rangle = | p + \hbar k \rangle $
We find
\begin{eqnarray}
\hat V^I  | p \rangle &= & - \frac{1}{2} \sum_{\rm L} | p + \hbar k_L \rangle \Omega_{\rm L}  e^{-i ( \delta_{\rm L}^{p+} t )} \label{Vinter} \\
\delta_{\rm L}^{p\pm} & =&  \omega_{\rm L} - (E_2-E_1)/\hbar -  \frac{k_{\rm L}}{m}(p   \pm \hbar k_{\rm L} /2 )  
\end{eqnarray}
where  $\hbar \Omega_{\rm L}(t) = \bm d. {\bm E}_{\rm L} e^{ - \Phi_{\rm L}(t)}$ and 
$\delta_{\rm L}^{p\pm} =  \delta_{\rm L}^0 + \delta_{\rm L}^{\rm D}(p) \pm \delta_{\rm L}^{\rm r}$:
The detuning $\delta_{\rm L}^0 = \omega_{\rm L} - (E_2-E_1)/\hbar $, the Doppler shift $ \delta_{\rm L}^{\rm D}(p) = -  k_{\rm L}. p /m $ and recoil frequency $ \delta_{\rm L}^{\rm r} = - \hbar k_{\rm L}^2 /2 m  $ appear naturally.




With $\hat \rho^I_{i j} = {\hat U_i}^\dag \hat \rho_{i j} {\hat U_j}$,  
the evolution reads as:

\begin{equation} \begin{pmatrix}
\frac{\partial \hat \rho_{11}^I }{\partial t}	 & 	\frac{\partial \hat \rho_{12}^I }{\partial t} \\ 
\frac{\partial \hat \rho_{21}^I }{\partial t} & 	\frac{\partial \hat \rho_{22}^I }{\partial t}
\end{pmatrix} = \frac{1}{i\hbar} \sum_{\rm L}
\begin{pmatrix}
{{\hat V} {}^I}^\dag \hat \rho_{21}^I - \hat \rho_{12 }^I \hat V^I   &  	{{\hat V} {}^I}^\dag \hat \rho_{22}^I - \hat \rho_{11}^I 	{{\hat V} {}^I}^\dag\\ 
{{\hat V} {}^I} \hat \rho_{11}^I - \hat \rho_{22}^I 	{{\hat V} {}^I}& 
{{\hat V} {}^I}\hat \rho_{12}^I - \hat \rho_{21 }^I 	{{\hat V} {}^I}^\dag
\end{pmatrix}
\end{equation}

Assuming there is no external field from now and using  $\displaystyle {\rho^I}_{i j }^{p' p} = \langle p' | \hat \rho_{i j }^I | p\rangle  = e^{i (p'^2-p^2) t/2m \hbar} e^{i (E_i-E_j) t/\hbar} \rho_{i j }^{p' p} $, the latter can be written as:


{\footnotesize
	\begin{equation}
	\begin{pmatrix}
	\frac{\partial   {\rho^I}_{11}^{p' p} }{\partial t}	 & 	\frac{\partial  {\rho^I}_{12}^{p' p} }{\partial t} \\ 
	\frac{\partial  {\rho^I}_{21}^{p' p} }{\partial t} & 	\frac{\partial  {\rho^I}_{22}^{p' p} }{\partial t}
	\end{pmatrix} = - \frac{1}{2 i} \sum_{\rm L}
	\begin{pmatrix}
	\Omega_{\rm L}^*	e^{i  \delta_{\rm L}^{p'+} t   }   {\rho^I}_{21}^{(p'+\hbar k_{\rm L})  p} -   \Omega_{\rm L} {\rho^I}_{12 }^{p' (p+\hbar k_{\rm L})}   e^{-i  \delta_{\rm L}^{p+} t   }    &  	 \Omega_{\rm L}^* e^{i  \delta_{\rm L}^{p'+} t   }   {\rho^I}_{22}^{(p'+\hbar k_{\rm L}) p} -  \Omega_{\rm L}^* {\rho^I}_{11}^{p' (p-\hbar k_{\rm L})}  e^{i  \delta_{\rm L}^{p-} t  } \\ 
	\Omega_{\rm L}	e^{-i  \delta_{\rm L}^{p'-} t   }   {\rho^I}_{11}^{(p'-\hbar k_{\rm L}) p} -  \Omega_{\rm L} {\rho^I}_{22}^{p' (p+\hbar k_{\rm L})}   e^{-i  \delta_{\rm L}^{p+} t   }  & 
	\Omega_{\rm L}	e^{-i  \delta_{\rm L}^{p'-} t  }  {\rho^I}_{12}^{(p'-\hbar k_{\rm L}) p} -  \Omega_{\rm L}^* {\rho^I}_{21 }^{p' (p-\hbar k_{\rm L})}  e^{i  \delta_{\rm L}^{p-} t   } 
	\end{pmatrix} \label{eq_density}
	\end{equation}
}

\subsubsection{Wigner function}

It is quite convenient to use
the so-called non-diagonal Wigner functions 
by defining $W_{i j}^I = W_{\hat \rho_{i j}^I}/h$ as the Wigner transform function associated to $ \hat \rho_{i j}^I = \langle i |\hat \rho^I | j\rangle$.
So
$ W_{i j}(r,p,t) = e^{i (E_j-E_i) t/\hbar} W_{i j}^I(r-p t/m,p,t)  
$ and the evolution equations become:



	\begin{eqnarray}
	\frac{\partial  W_{11}^I }{\partial t}	 
	(r,p,t) & =&   
	- \sum_{\rm L}
	\Im \left[   \Omega_L^* (r,p,t)
	W_{21}^I (r- \hbar k_{\rm L} t /2m,p+\hbar k_{\rm L}/2,t)
	\right] \label{int_wigner_a}
	\\
	\frac{\partial   W_{21}^I }{\partial t}  (r,p,t) & = &
	\frac{1}{2 i} \sum_{\rm L} \Omega_L(r,p,t) (W_{22}^I (r- \hbar k_{\rm L} t /2m,p+\hbar k_{\rm L}/2,t) -
	W_{11}^I (r+ \hbar k_{\rm L} t /2m,p-\hbar k_{\rm L}/2,t) 
	) 
	\label{int_wigner_b}
	\\	
	\frac{\partial 	W_{22}^I }{\partial t}
	(r,p,t)  & = & 
	\sum_{\rm L}
	\Im \left[   \Omega_L^*(r,p,t) W_{21}^I (r+ \hbar k_{\rm L} t /2m,p-\hbar k_{\rm L}/2,t)
	\right]
	\label{int_wigner_c}
	\end{eqnarray}

where 
\begin{equation}
\Omega_{\rm L}(r,p,t)  = \Omega_{\rm L} e^{i (k_L r   +  k_{\rm L} p t /m  -  \delta_{\rm L}^0 t   - \Phi_{\rm L}(t))	}
\label{Omega}
\end{equation}






\subsection{Single laser case (Bloch equation)}




When there is only one laser, we can define
%$ \tilde W_{21}^I = e^{-i (k_{\rm L} r   +  k_{\rm L} p t /m  -  \delta_{\rm L}^0 t  - \Phi_{\rm L} )} \bar W_{21}^I$

\begin{eqnarray*}
	\tilde W_{11}^I(r,p,t) &= &   W_{11}^I (r,p,t)  \\
	\tilde W_{22}^I (r,p,t)& =&   W_{22}^I (r- \hbar k_{\rm L} t /m,p+\hbar k_{\rm L},t) \\
	\tilde W_{21}^I (r,p,t) 	&= & e^{-i (k_{\rm L} r   + \frac{ k_{\rm L} p t}{m}  -  \delta_{\rm L}^0 t  - \Phi_{\rm L} )}  W_{21}^I (r- \frac{\hbar k_{\rm L} t}{ 2m},p+ \frac{\hbar k_{\rm L}}{2},t)
\end{eqnarray*}


If we assume $\Omega_{\rm L}$ real, the evolution is governed by


\begin{eqnarray}
	\frac{\partial   }{\partial t}	 
	\frac{
		\tilde	W_{11}^I  - \tilde W_{22}^I 
	}{2} & =&   
	-  \Omega_L \Im  
	\tilde W_{21}^I   + \frac{ \hbar k_{\rm L}}{ 2 m} \frac{\partial   }{\partial r}   \tilde W_{22}^I 
	\\
	\frac{\partial   }{\partial t}  \Re \tilde W_{21}^I & = & - 	\delta_{\rm L}^{p+}   \Im \tilde W_{21}^I -\frac{ \hbar k_{\rm L}}{  2m} \frac{\partial   }{\partial r}   \Re \tilde W_{21}^I
	\\
	\frac{\partial   }{\partial t}  \tilde \Im W_{21}^I & = & 	\delta_{\rm L}^{p+}  \Re \tilde W_{21}^I
	+
	\Omega_L 	\frac{\tilde W_{11}^I  - \tilde W_{22}^I }{2 }   -\frac{ \hbar k_{\rm L}}{  2m} \frac{\partial   }{\partial r}   \Im \tilde W_{21}^I
\end{eqnarray}

We recognize the standard Bloch equations except for the term in $\displaystyle \frac{ \hbar k_{\rm L}}{  2m} \frac{\partial   }{\partial r}$.
We can thus retrieve the Bloch equations from the exact Wigner function evolution by performing series expansion in $\hbar k$. 
This approach justifies the semi-classical equation for the particles evolution that we derive from heuristic considerations.

\section{Semi-classical evolution}
\label{Semiclassical evolution}


From the quantum evolution, we can derive the semi-classical evolution of the atomic motion. The underlying assumption is that
the displacement of the atom during the internal relaxation time is very small. The internal variables follow quasi-adiabatically the external motion \cite{dalibard1985atomic}. It is then possible to separate the internal and the external degree of freedom.

The Doppler or recoil effects, or the use of the stationary state of the Bloch equation can be done with hand-waving arguments  
(see for instance in Ref. \cite{2016PhRvA..93f3410H}). Nevertheless, the Lagrangian description (individual particles are followed through time), Eulerian description and interaction picture  that freeze the motion in the Eulerian description may  lead to confusion. We will clarify this distinction.





\subsection{Definition of a force}
\label{Force_Bloch}

For simplicity, we neglect the external potentials (but they can be included in the interaction picture if needed).


In the semi-classical approach, the particle motion is classical: for a given particle initially at $\bm r(t_0)=\bm r_0$ and  $\bm v(t_0)=\bm v_0$ at time $t=t_0$ its trajectory in phase space  $\bm r(t ),\bm p(t)=m \bm v(t)$ is given 
by Newton's equation of motion 
$\displaystyle m \frac{ d \bm v}{d t} (t)= \bm F(\bm r(t),\bm v(t), t)$.


The standard way to define the force in laser cooling is by using the Ehrenfest theorem 
(see for instance \cite{cohen1990atomic,Met1}, but other methods exists \cite{romanenko2017atoms,podlecki2017radiation,sonnleitner2017will}).
Knowing the light field seen by the atom at the position $\bm r$ with velocity $\bm v = \bm p/m$ enables to solve the optical Bloch equations (density matrix $\hat \sigma (t)$ evolution) to determine the atomic internal state.
The force is then derived from $\bm F = - tr[\hat \sigma(t )\bm \nabla \hat H] =\displaystyle   \langle \frac{\partial \bm d.\bm E}{\partial \bm r} \rangle $. The usual optical Bloch equations  where $\sigma_{i j } (t)$ stands for $ \sigma_{i j } (t; r_0, v_0, t_0)$ read as

	\begin{equation}
	\begin{pmatrix}
	\frac{\partial   {\sigma}_{11} }{\partial t}	 & 	\frac{\partial  {\sigma}_{12} }{\partial t} \\ 
	\frac{\partial  {\sigma}_{21} }{\partial t} & 	\frac{\partial  {\sigma}_{22} }{\partial t}
	\end{pmatrix} (t) = - \frac{ 1}{2 i} \sum_{\rm L}
	\begin{pmatrix}
	\Upomega_{\rm L}^*(r(t),t)   {\sigma}_{21}(t) -  \Upomega_{\rm L}(r(t),t) {\sigma}_{12 } (t)   &  	\Upomega_{\rm L}^*(r(t),t)  ({\sigma}_{22}(t) -  {\sigma}_{11} (t)) \\ 
	\Upomega_{\rm L}(r(t),t)(   {\sigma}_{11}(t) -  {\sigma}_{22} (t)  ) & 
	\Upomega_{\rm L}(r(t),t)  {\sigma}_{12} (t)-  \Upomega_{\rm L}^* (r(t),t) {\sigma}_{21 } (t)
	\end{pmatrix} 
	\label{OBE}
	\end{equation}

where  $\displaystyle \Upomega_{\rm L}(r,t) = 
\Upomega_{\rm L} e^{ i ( {\bm k}_{\rm L}. {\bm r}  - \omega_{\rm L} t  - \Phi_{\rm L} )}$.
The rapidly oscillating terms  can be removed by introducing slowly varying quantities as
$\displaystyle  \sigma_{i j}^I (t) = e^{-i (E_j-E_i) t/\hbar} \sigma_{i j}(t)$. 

%And finally, one retrieves the 
%The standard case of a single laser with rotating frame Bloch notations can be easily found using 
%$ {\tilde \sigma}_{2 1 }(t)  = {\sigma}_{2 1 }(t) e^{i ( \omega_{\rm L} - (E_2-E_1)) t/\hbar} $. 


The absence of Doppler shift in the expression of $\Upomega_{\rm L}(r,t)$ may be surprising, especially when  compared to Eq. (\ref{eq_density})  (using $p'=p=p(t)$, $r=r(t)$ and  $\hbar k_{\rm L}$ put to $0$). 
The explanation is the following: we use $\bm r (t)= \bm r (t; \bm r_0, \bm v_0, t_0)$ so the Lagrangian description where individual particles are followed through time, whereas, when dealing with the Wigner $W(\bm r, \bm v, t)$ or PSD $\rho(\bm r, \bm v, t)$ picture, we use in the Eulerian description. 
The connection between Lagrangian and Eulerian coordinates explains why the Doppler effect is correctly taken in both Eq.(\ref{OBE}) with
$\displaystyle  \Upomega_{\rm L}(r(t),t) = 
\Upomega_{\rm L} e^{ i ( {\bm k}_{\rm L}. {\bm r(t)}  - \omega_{\rm L} t  - \Phi_{\rm L}(t) )} $,
and in 
Eq. (\ref{eq_density})
with	
$\displaystyle 
\Omega_{\rm L}(r,p,t)  = \Omega_{\rm L} e^{i (k_L r   +  k_{\rm L} p t /m  -  \delta_{\rm L}^0 t   - \Phi_{\rm L}(t))	}$. In any case, the instantaneous laser phase seen by the atoms is correct, including the Doppler effect because $\displaystyle  \frac{d r(t)}{d t} = p(t)  /m$.


Similarly,  in the Eulerian description the force  is thus given by $\displaystyle  {\rm Tr}[\hat \sigma(t )\bm \nabla \hat H]$, or $\displaystyle  {\rm Tr}[\hat \rho(t )^I \bm \nabla \hat V^I]$
using  the cyclic invariant of the  trace. We have
$\displaystyle  V^I(r,p,t) = - \sum_{\rm L} \frac{\hbar}{2} \Omega_{\rm L}(r,p,t)$ so
$\bm \nabla V^I(r,p,t) = \displaystyle 	 - i\sum_{\rm L} \frac{\hbar \bm k_{\rm L} }{2} \Omega_{\rm L}(r,p,t)$.

So in conclusion and back to our Lagrangian description we have:
\begin{equation}
\bm F (\bm r(t),\bm v(t), t) =\Im \left[ {\sigma}_{2 1 }(t)   	\sum_{\rm L} \hbar \bm k_{\rm L} \Omega_{\rm L}^*(\bm r(t),t)\right]
\label{force} 
\end{equation}
As we chose plane waves  (or $ \bm \nabla  E_{\rm L}=0$), there is no direct dipolar force. Also, because of the interplay between the Bloch equations (Eq.\ref{OBE}) and the force (Eq.\ref{force}), the
atomic velocity $\bm v(t )$ and position $\bm r(t )$ should be updated in a short time
interval (typically ps), and the calculation of the Bloch equation evolution iterated on a similar 
time scale 	
\cite{2016PhRvA..93f3410H}.





\subsection{Phase space evolution equation}
\label{Force_Wigner}

Here, we would like to justify the equations we just derived assuming a separation of the external and internal degrees of freedom.
However, we know that without spontaneous emission, this is valid 
only if the ratio of resonant photon momentum to atomic momentum dispersion is small $\hbar k/\Delta p \ll 1$. In such a case, 
the rapid processes acting on  the internal degrees of
freedom can be separated from the slow processes associated
with translational motion.
 The dynamics of the atomic ensemble is thus
determined by the slow change of the distribution function
in translational degrees of freedom $w(r, p)= W_{11}+W_{22}$ and 
the expansion in $\hbar k$, that we will derive here for completeness, is justified  \cite{dalibard1985atomic}. 


One analogue of the classical phase space distribution
$\rho$ is
the total distribution function
in translational degrees of freedom, $w(r, p,t)$ as plotted in \cite[Fig. 2(b)]{main_art}.
Equations (\ref{Wigner_eq_brute_1}-\ref{Wigner_eq_brute_4}) (written for simplicity without the external potentials), become:
{\footnotesize
	\begin{eqnarray}
	\left[ \frac{\partial   }{\partial t}	 
	+\frac{ p}{m} \frac{\partial }{\partial  r}   
	\right]W_{11}(r,p,t) & =&   
	-
	\frac{1}{2 i} \sum_{\rm L} ( \Upomega_L^* (r,t)
	W_{21} (r,p+\hbar k_{\rm L}/2,t) - \Upomega_L (r,t) W_{12} (r,p+\hbar k_{\rm L}/2,t)
	) \label{eq_Wigner1}
	\\
	\left[	\frac{\partial   }{\partial t}+\frac{ p}{m}  \frac{\partial }{\partial  r} 
	-
	\frac{E_1 - E_2}{i\hbar}	
	\right] W_{12}(r,p,t) & = &
	-
	\frac{1}{2 i} \sum_{\rm L} \Upomega_L^* (r,t) (
	W_{2 2} (r,p+\hbar k_{\rm L}/2,t) - W_{11} (r,p-\hbar k_{\rm L}/2,t)
	) \label{eq_Wigner2}
	\\
	\left[	\frac{\partial   }{\partial t}  +\frac{ p}{m}  \frac{\partial }{\partial  r} 
	+
	\frac{E_1 - E_2}{i\hbar}
	\right] W_{21}(r,p,t) & = &
	-
	\frac{1}{2 i} \sum_{\rm L} \Upomega_L (r,t) (
	W_{11} (r,p-\hbar k_{\rm L}/2,t) - W_{22} (r,p+\hbar k_{\rm L}/2,t)
	) \label{eq_Wigner3}
	\\	
	\left[	\frac{\partial  }{\partial t}
	+\frac{ p}{m}  \frac{\partial }{\partial  r}   
	\right]   W_{22} (r,p,t)  & = & 
	- \frac{1}{2 i} \sum_{\rm L} ( \Upomega_L (r,t)
	W_{12} (r,p-\hbar k_{\rm L}/2,t) - \Upomega_L^* (r,t) W_{21} (r,p-\hbar k_{\rm L}/2,t)
	) \label{eq_Wigner4}
	\end{eqnarray}
}
with  
$\hbar \Upomega_{\rm L}(r,t) = 
\bm d. {\bm E}_{\rm L} e^{ i ( {\bm k}_{\rm L}. {\bm r}  - \omega_{\rm L} t  - \Phi_{\rm L} )} $. 


An frequently used method to derive a continuity equation
as \cite[Eq.(1)]{main_art} for $\rho = w$
is to
expand  the Wigner distribution equations
in a power series of
the photon momentum $\hbar k$
\cite{minogin1987laser,kazantsev1990mechanical,dalibard1985atomic,1986RvMP...58..699S,1991JOSAB...8.1341Y,2003JETP...96..383B,2013JETP..117..222P}.
In the presence of spontaneous emission, the second order  leads to the standard
Fokker-Planck equation 	\cite{minogin1987laser,kazantsev1990mechanical,dalibard1985atomic,1986RvMP...58..699S,1991JOSAB...8.1341Y,2003JETP...96..383B,2013JETP..117..222P}. 
The simplest formulation is restricted to the first order approximation, therefore
$\displaystyle W_{21} (r ,p \mp \hbar k_{\rm L}/2,t) \approx	 W_{21} (r,p,t) \mp \frac{\hbar k_{\rm L}}{2}  \frac{\partial    }{\partial p}
\tilde W_{21} (r,p,t)$.
To this first order in $\hbar k_{\rm L}$, the sum of
(\ref{eq_Wigner1}) and (\ref{eq_Wigner4}) is:
%\begin{widetext}
	\begin{equation}
	\left[	\frac{\partial   }{\partial t}  +\frac{ p}{m}  \frac{\partial }{\partial  r} 
	\right]
	w(r,p,t)  =   
	-  \sum_{\rm L}
	\Im \left[   \Omega_L^* (r,t) 
	\hbar k_{\rm L}  \frac{\partial    }{\partial p}
	W_{21} (r,p,t)
	\right]
	\label{wigner_first_order}
	\end{equation}
%\end{widetext}



Since the recoil momentum $\hbar k$ is small, the variation of
atomic translational motion is slower than the atomic internal state change. The latter follows the varying
translational state 	$w(r,p,t) $  \cite{minogin1984dynamics}.
Fast relaxation of the internal atomic state means that, the functions
$W_{ij} (r,p,t)$ follow the distribution function
$w(r,p,t) $. %So 	$W_{ij} (r,p,t) \simeq W_{ij}^0 (r,p,t) w(r,p,t)  $.
%Alternatively, following the optical Bloch equations point of view;  the internal states amplitudes  $ W_{ij}^0 (r,p,t)$ are decoupled from the external ones $ w (r,p,t)$. So, $ w (r,p,t)$ represents only the  probability of presence, the internal state population and coherences being represented by $ W_{ij}^0 (r,p,t)$. 


At zero order in $\hbar k_{\rm L}$ we  have the simplest approximation
$W_{ij} (r,p,t) \approx W_{ij}^0 (r,p,t) w(r,p,t)$.
Eq.(\ref{wigner_first_order}) leads to
\begin{equation}
\left[	\frac{\partial   }{\partial t}  +\frac{ p}{m}  \frac{\partial }{\partial  r} 
\right]
w(r,p,t)  =  - \frac{\partial   [ F ( r  ,  p, t)  w(r,p,t)] }{\partial p}
\end{equation}
We recognize a continuity equation as \cite[Eq.(1)]{main_art} with the force given by
\begin{equation} F ( r, p, t) =\Im \left[ W_{2 1 }^0( r, p,t)   	\sum_{\rm L} \hbar  k_{\rm L} \Omega_{\rm L}^* ( r,t)\right]
\label{force_wigner}
\end{equation}
So in a classical picture, this expression of the force shall be used to calculate individual particles trajectories.


The evolution of the Wigner function is given by Eqs.(\ref{eq_Wigner1})-(\ref{eq_Wigner4}), with 	$W_{ij} (r,p,t) \approx W_{ij}^0 (r,p,t) w(r,p,t)$, to obtain
\begin{widetext}
	\begin{eqnarray}	 
	\frac{\partial W_{11}^0(r+p t /m,p,t)  }{\partial t}	 & =&   
	- \sum_{\rm L}
	\Im \left[   	\Omega_{\rm L}^*(r+p t /m,t) 
	W_{21}^0 (r+p t /m,p,t)
	\right] 
	\\
	\frac{\partial W_{21}^0(r+p t /m,p,t)  }{\partial t}    & = &
	\frac{1}{2 i} \sum_{\rm L} 	\Omega_{\rm L}(r+p t /m,t)  (W_{22}^0(r+p t /m,p,t) -
	W_{11}^0 (r+p t /m,p,t)
	) \\	
	\frac{\partial 	W_{22}^0 (r+p t /m,p,t)  }{\partial t}
	& = & 
	\sum_{\rm L}
	\Im \left[   	\Omega_{\rm L}^*(r+p t /m,t)  W_{21}^0 (r+p t /m,p,t)
	\right]
	\end{eqnarray}
\end{widetext}
where we have used
$\displaystyle	\left[ \frac{\partial   }{\partial t}	 
+\frac{ p}{m} \frac{\partial }{\partial  r}   
\right]W_{11}^0(r+p t /m,p,t) = 		\frac{\partial W_{11}^0(r+p t /m,p,t)  }{\partial t}$.	

We partially recognize the optical Bloch equations  (Eqs.\ref{OBE}), with $\sigma_{i j}(t) = 	W_{ij}^0 (r_0+p_0 t /m,p_0,t)$ \cite{dalibard1985atomic}. 
This is the usual   first order in time 
connection between  Lagrangian and Eulerian specification:
$\bm r (t)= \bm r (t; \bm r_0, \bm v_0, t_0) \approx r_0+v_0 t $,  $p(t) \approx p_0$.
So  to first order $\sigma_{i j}(t) \approx 	W_{ij}^0 (r( t),p(t),t)$ and
the force given by Eq.(\ref{force_wigner})  is exactly the same force as Eq.(\ref{force}). 

An alternative way to derive these expressions consists in using the interaction picture. A similar method using $w^I(r, p,t) = W_{11}^I+W_{22}^I$  
$W_{ij}^I (r,p,t) \approx {W_{ij}^I}^0 (r,p,t) w(r,p,t)$
from
Eqs.(\ref{int_wigner_a})-(\ref{int_wigner_c}) leads, to first order in $\hbar k_{\rm L}$ to:
\begin{widetext}
	\begin{eqnarray}	 
	\frac{\partial {W_{11}^I}^0  }{\partial t} (r,p,t)	 & =&   
	- \sum_{\rm L}
	\Im \left[   	\Omega_{\rm L}^*(r,p,t) 
	{W_{21}^I}^0 (r,p,t)
	\right] 
	\\
	\frac{\partial {W_{21}^I}^0  }{\partial t} (r,p,t)   & = &
	\frac{1}{2 i} \sum_{\rm L} 	\Omega_{\rm L}(r,p,t)  ({W_{22}^I}^0(r,p,t) -
	{W_{11}^I}^0 (r,p,t)
	) \\	
	\frac{\partial 	{W_{22}^I}^0   }{\partial t}(r,p,t)
	& = & 
	\sum_{\rm L}
	\Im \left[   	\Omega_{\rm L}^*(r,p,t)  {W_{21}^I}^0 (r,p,t)
	\right]
	\end{eqnarray}
\end{widetext}
which are the usual Bloch equations in the particle frame. The Doppler effect is here explicitly included. Indeed, the continuity equation reads as
\begin{equation*}
\frac{\partial w^I  }{\partial t}	 
(r,p,t)  = -
\left[
- \frac{ t}{m} \frac{\partial    }{\partial r} 	 +  \frac{\partial    }{\partial p}\right] \left( F^I ( r, p, t) w^I(r,p,t) \right)  
\end{equation*}
for the force 
$F(\bm r + \bm p t /m,\bm p,t) = F^I ( r, p, t) =	\sum_{\rm L} \hbar k_{\rm L}   \Omega_L^* (r,p,t)
W_{21}^I (r,p,t)^0$.

This is indeed the classical continuity equation \cite[Eq.(1)]{main_art}. In the interaction picture 
$\rho(\bm r,\bm p,t) = \rho^I(\bm r-\bm p t /m,\bm p,t)$ leads to
\begin{equation}
\frac{\partial  \rho^I}{\partial t} (\bm r,\bm p,t)  + \left[
- \frac{ t}{m} \frac{\partial    }{\partial \bm r} 	 +  \frac{\partial    }{\partial \bm p}\right]   (\rho^I F^I)(\bm r,\bm p,t) = 0 \label{rho_rep_int}
\end{equation}
where 	$F(\bm r,\bm p,t) = F^I(\bm r-\bm p t /m,\bm p,t)$.








